Conflict-Aware Replicated Data Types

We introduce Conflict-Aware Replicated Data Types (CARDs). CARDs are significantly more expressive than Conflict-free Replicated Data Types (CRDTs) as they support operations that can conflict with each other. Introducing conflicting operations typically brings the need to block an operation in at least some executions, leading to difficulties in programming and reasoning about correctness, as well as potential inefficiencies in implementation. The salient aspect of CARDs is that they allow ease of programming and reasoning about programs comparable to CRDTs, while enabling algorithmic inference of conflicts so that an operation is blocked only when necessary. The key idea is to have a language that allows associating with each operation a two-state predicate called {\em consistency guard} that relates the state of the replica on which the operation is executing to a global state (which is never computed). The consistency guards bring three advantages. First, a programmer developing an operation needs only to choose a consistency guard that states what the operation will rely on. In particular, they do not need to consider the operation conflicts with other operation. This allows purely {\em modular reasoning}. Second, we show that consistency guard allow reducing the complexity of reasoning needed to prove invariants that hold as CARD operations are executing. The reason is that consistency guard allow reducing the reasoning about concurrency among operations to purely {\em sequential reasoning}. Third, conflicts among operations can be algorithmically inferred by checking whether the effect of one operation preserves the consistency guard of another operation.

==> fig-hoare-rules.tex <==
% Hoare-style rules for CARDs
%
\begin{mathpar}
\vspace{-1ex}
  \inferrule*[Left=UseGuard]{
    \triple{P \land g}{\OLDSTORE := \STORE; o}{Q}
  }{
    \triple{P}{ \operc{g}{o} }{Q}
  }
% \vspace{-2ex}
\end{mathpar}
%
%
%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> fig-model-comparison.tex <==

\tiny
\begin{tabular}{p{3cm} p{3cm} p{3cm} p{3cm}}
  {\small CARDs} & {\small CRDTs} & {\small RedBlue} & \small{\cite{Gotsman:2016}} \\
  \hline
  Non-commutative effects & Only commutative effects & Non-commutative effects & Non-commutative effects \\
  Minimal coordination for each operation pair & No coordination & Two coordination classes & Minimal coordination for each operation pair \\
  Ensures application invariants & Application invariants left to user & Ensures application invariants & Ensures application invariants \\
  Conflict inference from guards & No conflicts & Conflicts prevented by specifying coordination class & Conflicts specified by tokens \\
  One-operation reasoning & One-operation reasoning & Operations must be reasoned about together & Operation-pair reasoning \\
  Sequential reasoning & Sequential reasoning & Concurrent reasoning & Sequential reasoning for proving correctness, concurrent reasoning for identifying conflicts \\
  Realtime strengthening of coordination (via nested guards) & N/A & Predefined coordination & Predefined coordination
\end{tabular}

